Single Image Test-Time Adaptation for Segmentation

Test-Time Adaptation (TTA) methods improve the robustness of deep neural networks to domain shift on a variety of tasks such as image classification or segmentation. This work explores adapting segmentation models to a single unlabelled image with no other data available at test-time. In particular, this work focuses on adaptation by optimizing self-supervised losses at test-time. Multiple baselines based on different principles are evaluated under diverse conditions and a novel adversarial training is introduced for adaptation with mask refinement. Our additions to the baselines result in a 3.51 and 3.28 % increase over non-adapted baselines, without these improvements, the increase would be 1.7 and 2.16 % only.

==> figures/coco/coco_error_reduction_per_sev_dist.tex <==
\begin{figure*}[tb]
    \centering
        \includegraphics[keepaspectratio, width=\linewidth]{plots/coco/total_error_reduction_per_severity_per_kind.png}
    \caption{Comparison of total error reduction across methods per corruption levels on COCO-C dataset for optimal hyperparameters for each corruption kind and severity. Different \ac{tta} hyper-parameters are used for each corruption and severity combination.}
    \label{fig:coco:sev_barplot_hparams_each}
\end{figure*}

==> figures/coco/test_voc.tex <==
\begin{figure} [tbh]
    \centering
        \includegraphics[keepaspectratio, width=1\linewidth]{plots/test_datasets_voc_miou_red_per_im.png}
    \caption{\ac{tta} $\text{m}\overline{\text{IoU}}_i$ error reduction (\%) of COCO model on the VOC test dataset with hyper-parameters selected on COCO-C.
    }
    \label{fig:coco:test_voc}
\end{figure}


==> figures/coco/tta_miou_tta_ent.tex <==
\begin{figure}[bth]
    \centering
        \includegraphics[keepaspectratio, width=0.93\linewidth]{plots/coco/per_image_miou_ent_delta_comp.png}
    \caption{The relationship between per-image non-adapted (NA) prediction entropy and \ac{tta} $\text{m}\overline{\text{IoU}}_i$ improvement on the COCO-C dataset. The difference between NA $\text{m}\overline{\text{IoU}}_i$ and the \ac{tta} $\text{m}\overline{\text{IoU}}_i$ is shown ($\text{m}\overline{\text{IoU}}_i \Delta$). Least-squares line fitted to the points in yellow.}
    \label{fig:coco:miou_ent_tta}
\end{figure}

==> figures/gta5/error_reduction_per_sev_dist.tex <==
\begin{figure*}[bt]
    \centering
        \includegraphics[keepaspectratio, width=\linewidth]{plots/gta5/total_error_reduction_per_severity_per_kind.png}
    \caption{Comparison of total error reduction across methods per corruption levels on GTA5-C dataset. Different \ac{tta} hyper-parameters are used for each corruption and severity combination.}
    \label{fig:gta5:sev_barplot_hparams_each}
\end{figure*}

==> figures/gta5/tta_miou_tta_ent.tex <==


\begin{figure}[bth]
    \centering
        \includegraphics[keepaspectratio, width=0.93\linewidth]{plots/gta5/per_image_miou_ent_delta_comp.png}
    \caption{The relationship between per-image non-adapted (NA) prediction entropy and \ac{tta} $\text{m}\overline{\text{IoU}}_i$ improvement on the GTA5-C dataset. The difference between NA $\text{m}\overline{\text{IoU}}_i$ and the \ac{tta} $\text{m}\overline{\text{IoU}}_i$ is shown ($\text{m}\overline{\text{IoU}}_i \Delta$). Least-squares line fitted to the points in yellow.}
    \label{fig:gta5:miou_ent_tta}
\end{figure}


==> figures/teaser.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cccc}
        image &  ground truth & NA & TTA \\
        \includegraphics[width=0.24\linewidth]{images/teaser_images/orig_im.png}
         & 
         \includegraphics[width=0.24\linewidth]{images/teaser_images/gt.png}
         &
         \includegraphics[width=0.24\linewidth]{images/teaser_images/it_0.jpg}
         &
         \includegraphics[width=0.24\linewidth]{images/teaser_images/it_5.jpg}
         \\
    \end{tabular}
    
    \caption{Non-adapted (NA) and adapted (TTA) masks.}
    \label{fig:teaser}
\end{table}


%     \subfloat[Original Image]{
    %     \label{ref_label1}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/orig_im.png}
    % }
    % \subfloat[Iteration 0]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_0.jpg}
    % }
    % \subfloat[Iteration 1]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_1.jpg}
    % }
    % \subfloat[Iteration 2]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_2.jpg}
    % }
    % \subfloat[Iteration 3]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_3.jpg}
    % }
    % \subfloat[Iteration 4]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_4.jpg}
    % }
    %  \subfloat[Iteration 5]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/it_5.jpg}
    % }
    % \subfloat[GT]{
    %     \label{ref_label2}
    %     \includegraphics[width=0.5\textwidth]{images/teaser_images/gt.png}
    % }

==> tables/acdc/tta_results.tex <==
\begin{table*}[h]
    \setlength{\tabcolsep}{4pt}
    \centering
        \begin{tabular}{lrrrrrrrrrrrr}
            \toprule
            TTA method: & \multicolumn{2}{c}{ENT} & \multicolumn{2}{c}{PL} & \multicolumn{2}{c}{ADV} & \multicolumn{2}{c}{AugCo} & \multicolumn{2}{c}{IoU} & \multicolumn{2}{c}{REF} \\ 
            \midrule
norm only: & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark}  & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} \\


\midrule
$\Delta_{\text{ABS}}$ & 0.35 & 1.05 & 0.28 & 0.36 & 0.07 & - & 0.39 & 0.16 & 0.06 & 0.07 & 1.41 & 5.96 \\
$\Delta_{\text{CORR}}$ & 1.40 & 8.65 & 1.14 & 1.44 & 0.28 & - & 1.59 & 0.65 & - & - & 5.69 & 24.09  \\
$\Delta_{\text{TOTAL}}$ & 0.52 & 1.96 & 0.42 & 0.54 & 0.11 & - & 0.59 & 0.24 & - & - & 2.12 & 8.99  \\
\bottomrule


\end{tabular}

\caption{Mean \ac{iou} improvements of different \ac{tta} methods on the ACDC test sets, relative to the non-adapted score of --- \%. 
}
\label{tab:sem_seg:gta5c:valid_agg}
\end{table*}

% & \multicolumn{2}{c}{IoU} & \multicolumn{3}{c}{error difference} & \multicolumn{2}{c}{best setting} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} 
% TTA method &  initial &  best &  abs & base (\%) & total (\%) & it&  lr\\

==> tables/gta5c/valid_summary_backup.tex <==
\begin{table*}[h]
    \setlength{\tabcolsep}{4pt}
    \centering
\begin{tabular}{l|rr|rrrr|rrrr|rrrr|rr|rr}
\toprule
 & \multicolumn{2}{c}{Ent} & \multicolumn{4}{c}{PL} & \multicolumn{4}{c}{Ref} & \multicolumn{4}{c}{AugCo} & \multicolumn{2}{c}{Adv} & \multicolumn{2}{c}{IoU} \\
\midrule
norm only & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c}{\tikzxmark} & \multicolumn{1}{c}{\checkmark} \\


loss & \multicolumn{1}{c}{ent} & \multicolumn{1}{c|}{ent} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c}{iou} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c|}{iou} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c}{iou} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c|}{iou} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c}{iou} & \multicolumn{1}{c}{ce} & \multicolumn{1}{c|}{iou} & \multicolumn{1}{c}{kl} & \multicolumn{1}{c|}{kl} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\


\midrule
$\Delta_{\text{ABS}}$ & 0.35 & 1.05 & 0.30 & 0.36 & 0.07 & 0.06 & 0.06 & 0.08 & 0.06 & 0.07 & 1.41 & 5.96 \\
$\Delta_{\text{CORR}}$ & 1.40 & 8.65 & 1.23 & 1.44 & 0.28 & 0.22 & 0.23 & 0.33 & - & - & 5.69 & 24.09  \\
$\Delta_{\text{TOTAL}}$ & 0.52 & 1.96 & 0.46 & 0.54 & 0.11 & 0.08 & 0.09 & 0.09 & - & - & 2.12 & 8.99  \\
\bottomrule
\end{tabular}

%   0.06 & 0.22 & 0.08


\caption{Mean \ac{iou} improvements of different \ac{tta} methods on the GTA5-C dataset, relative to the non-adapted score of 33.66 \%. The results are aggregated across all corruption types and severities, including no corruption. The methods are evaluated in two setups: Updating learnable parameters of normalization layers only and updating all the learnable network parameters. \ac{tta_ref} outperforms all other baselines in both setups.
}
\label{tab:sem_seg:gta5c:valid_agg}
\end{table*}

% & \multicolumn{2}{c}{IoU} & \multicolumn{3}{c}{error difference} & \multicolumn{2}{c}{best setting} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} 
% TTA method &  initial &  best &  abs & base (\%) & total (\%) & it&  lr\\
